Low-Rank Principal Eigenmatrix Analysis

Sparse PCA is a widely used technique for high-dimensional data analysis. In this paper, we propose a new method called low-rank principal eigenmatrix analysis. Different from sparse PCA, the dominant eigenvectors are allowed to be dense but are assumed to have a low-rank structure when matricized appropriately. Such a structure arises naturally in several practical cases: Indeed the top eigenvector of a circulant matrix, when matricized appropriately is a rank-1 matrix. We propose a matricized rank-truncated power method that could be efficiently implemented and establish its computational and statistical properties. Extensive experiments on several synthetic data sets demonstrate the competitive empirical performance of our method.

==> main.tex <==
%%
%%  main part
%%

\section{Introduction}  \label{sec:introduction}

\section{Model} \label{sec:model}

\section{Estimation} \label{sec:estimation}

\section{Theoretical Properties} \label{sec:theory}

\section{Empirical Analysis} \label{sec:empirical}

\subsection{Synthetic Data} \label{subsec:synthetic}

\subsection{Real Data} \label{subsec:real}

